Primal-dual stochastic gradient method for convex programs with many functional constraints

Stochastic gradient method (SGM) has been popularly applied to solve optimization problems with objective that is stochastic or an average of many functions. Most existing works on SGMs assume that the underlying problem is unconstrained or has an easy-to-project constraint set. In this paper, we consider problems that have a stochastic objective and also many functional constraints. For such problems, it could be extremely expensive to project a point to the feasible set, or even compute subgradient and/or function value of all constraint functions. To find solutions of these problems, we propose a novel (adaptive) SGM based on the classical augmented Lagrangian function. Within every iteration, it inquires a stochastic subgradient of the objective, and a subgradient and the function value of one randomly sampled constraint function. Hence, the per-iteration complexity is low. We establish its convergence rate for convex problems and also problems with strongly convex objective. It can achieve the optimal $O(1/\sqrt{k})$ convergence rate for convex case and nearly optimal $O\big((\log k)/k\big)$ rate for strongly convex case. Numerical experiments on a sample approximation problem of the robust portfolio selection and quadratically constrained quadratic programming are conducted to demonstrate its efficiency.

==> macros.tex <==
\usepackage{mathtools}
%\mathtoolsset{showonlyrefs}

%% macros for editing and commenting
\usepackage[normalem]{ulem} % to use \sout
\newcommand{\remove}[1]{{\color{Gray}\sout{#1}}}
\newcommand{\revise}[1]{{\color{blue}#1}}
\newcommand{\comm}[1]{{\color{red}(yx: #1)}}

\newcommand{\bm}[1]{\boldsymbol{#1}}


%% macros for vectors
\newcommand{\va}{{\mathbf{a}}}
\newcommand{\vb}{{\mathbf{b}}}
\newcommand{\vc}{{\mathbf{c}}}
\newcommand{\vd}{{\mathbf{d}}}
\newcommand{\ve}{{\mathbf{e}}}
\newcommand{\vf}{{\mathbf{f}}}
\newcommand{\vg}{{\mathbf{g}}}
\newcommand{\vh}{{\mathbf{h}}}
\newcommand{\vi}{{\mathbf{i}}}
\newcommand{\vj}{{\mathbf{j}}}
\newcommand{\vk}{{\mathbf{k}}}
\newcommand{\vl}{{\mathbf{l}}}
\newcommand{\vm}{{\mathbf{m}}}
\newcommand{\vn}{{\mathbf{n}}}
\newcommand{\vo}{{\mathbf{o}}}
\newcommand{\vp}{{\mathbf{p}}}
\newcommand{\vq}{{\mathbf{q}}}
\newcommand{\vr}{{\mathbf{r}}}
\newcommand{\vs}{{\mathbf{s}}}
\newcommand{\vt}{{\mathbf{t}}}
\newcommand{\vu}{{\mathbf{u}}}
\newcommand{\vv}{{\mathbf{v}}}
\newcommand{\vw}{{\mathbf{w}}}
\newcommand{\vx}{{\mathbf{x}}}
\newcommand{\vy}{{\mathbf{y}}}
\newcommand{\vz}{{\mathbf{z}}}

%% macros for matrices
\newcommand{\vA}{{\mathbf{A}}}
\newcommand{\vB}{{\mathbf{B}}}
\newcommand{\vC}{{\mathbf{C}}}
\newcommand{\vD}{{\mathbf{D}}}
\newcommand{\vE}{{\mathbf{E}}}
\newcommand{\vF}{{\mathbf{F}}}
\newcommand{\vG}{{\mathbf{G}}}
\newcommand{\vH}{{\mathbf{H}}}
\newcommand{\vI}{{\mathbf{I}}}
\newcommand{\vJ}{{\mathbf{J}}}
\newcommand{\vK}{{\mathbf{K}}}
\newcommand{\vL}{{\mathbf{L}}}
\newcommand{\vM}{{\mathbf{M}}}
\newcommand{\vN}{{\mathbf{N}}}
\newcommand{\vO}{{\mathbf{O}}}
\newcommand{\vP}{{\mathbf{P}}}
\newcommand{\vQ}{{\mathbf{Q}}}
\newcommand{\vR}{{\mathbf{R}}}
\newcommand{\vS}{{\mathbf{S}}}
\newcommand{\vT}{{\mathbf{T}}}
\newcommand{\vU}{{\mathbf{U}}}
\newcommand{\vV}{{\mathbf{V}}}
\newcommand{\vW}{{\mathbf{W}}}
\newcommand{\vX}{{\mathbf{X}}}
\newcommand{\vY}{{\mathbf{Y}}}
\newcommand{\vZ}{{\mathbf{Z}}}

\newcommand{\vlam}{{\bm{\lambda}}}
\newcommand{\vtheta}{{\bm{\theta}}}
\newcommand{\veta}{{\bm{\eta}}}
\newcommand{\vell}{{\bm{\ell}}}


%% macros for sets
\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cJ}{{\mathcal{J}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cO}{{\mathcal{O}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cQ}{{\mathcal{Q}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\cZ}{{\mathcal{Z}}}


%
\newcommand{\vareps}{\varepsilon}

%% macros for the real and imaginary parts
\newcommand{\ri}{{\mathrm{i}}}
\newcommand{\rr}{{\mathrm{r}}}

%% macros for math notions and operators
\newcommand{\EE}{\mathbb{E}} % expectation
\newcommand{\VV}{\mathbb{V}} % variance
\newcommand{\RR}{\mathbb{R}} % real
\newcommand{\CC}{\mathbb{C}} % complex
\newcommand{\ZZ}{\mathbb{Z}} % integer
\renewcommand{\SS}{{\mathbb{S}}} % symmetric matrix
\newcommand{\SSp}{\mathbb{S}_{+}} % symmetric positive semi-definite matrix
\newcommand{\SSpp}{\mathbb{S}_{++}} % symmetric positive definite matrix
\newcommand{\sign}{\mathrm{sign}} % sign function
\newcommand{\vzero}{\mathbf{0}} % 0 vector
\newcommand{\vone}{{\mathbf{1}}} % 1 vector

\newcommand{\dist}{\mathrm{dist}}    % distance
\newcommand{\op}{{\mathrm{op}}} % subscript for operator norm
\newcommand{\opt}{{\mathrm{opt}}} % subscript for optimal solution
%\newcommand{\supp}{{\mathrm{supp}}} % support
\newcommand{\Prob}{{\mathrm{Prob}}} % probability
\newcommand{\prox}{{\mathbf{prox}}} % proximal map
\newcommand{\Diag}{{\mathrm{Diag}}} % vector -> diagonal matrix
%\newcommand{\diag}{{\mathrm{diag}}} % matrix diagonal -> vector
\newcommand{\dom}{{\mathrm{dom}}} % domain
%\newcommand{\rank}{\textnormal{rank}}
%\newcommand{\grad}{{\nabla}}    % gradient
\newcommand{\tr}{{\mathrm{tr}}} % trace
\newcommand{\TV}{{\mathrm{TV}}} % total variation
\newcommand{\Proj}{{\mathrm{Proj}}} % projection
\newcommand{\Null}{{\mathrm{Null}}} % null space
\newcommand{\Dim}{{\mathrm{dim}}} % dimension
\newcommand{\etal}{{\textit{et al.}}}
\newcommand{\conj}{{\mathrm{conj}}} % conjugate
\newcommand{\vvec}{{\mathrm{vec}}}
\newcommand{\fold}{{\mathbf{fold}}} % fold into a tensor
\newcommand{\unfold}{{\mathbf{unfold}}} % unfold a tensor
\newcommand{\fit}{{\mathrm{fit}}} % data fitting
\newcommand{\obj}{{\mathrm{obj}}} % data fitting
\newcommand{\round}{{\mathrm{round}}}
\newcommand{\Var}{{\mathrm{Var}}}
% rounding number
\newcommand{\err}{{\mathrm{err}}}
\newcommand{\ST}{\mbox{ subject to }}
\newcommand{\st}{\mbox{ s.t. }}

\newcommand{\ip}[2]{\langle #1 , #2 \rangle}
\newcommand{\by}{{\bf y}}
\newcommand{\bxs}{{\bf x}_{\epsilon,\lambda,q}}
\newcommand{\od}{\frac{d}{dt}}
\newcommand{\pd}{{\partial }}
\newcommand{\rankk}{{\hbox{rank}}}




\newcommand{\prev}{{\mathrm{prev}}} % previous iteration

\DeclareMathOperator{\shrink}{shrink} % shrinkage
\DeclareMathOperator{\hardthr}{hardthr} % hard thresholding
\DeclareMathOperator*{\argmin}{arg\,min} % argmin
\DeclareMathOperator*{\argmax}{arg\,max} % argmax

\DeclareMathOperator*{\Min}{minimize}
\DeclareMathOperator*{\Max}{maximize}



%% macros for environments math equations

\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}

\newcommand{\bdm}{\begin{displaymath}}
\newcommand{\edm}{\end{displaymath}}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\bfl}{\begin{flushleft}}
\newcommand{\efl}{\end{flushleft}}

\newcommand{\bt}{\begin{tabbing}}
\newcommand{\et}{\end{tabbing}}

\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}

\newcommand{\beqs}{\begin{align*}} % no equation numbers
\newcommand{\eeqs}{\end{align*}}  % no equation numbers

%% macros for theorem-like environments

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{acknowledgement}{Acknowledgement}[section]
%\newtheorem{axiom}{Axiom}[section]
%\newtheorem{algorithm}{Algorithm}[section]
%\newtheorem{case}{Case}[section]
\newtheorem{claim}{Claim}[section]
%\newtheorem{conclusion}{Conclusion}[section]
%\newtheorem{condition}{Condition}[section]
%\newtheorem{conjecture}{Conjecture}[section]
%\newtheorem{corollary}{Corollary}[section]
%\newtheorem{criterion}{Criterion}[section]
%\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]
%\newtheorem{exercise}{Exercise}[section]
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{notation}{Notation}[section]
%\newtheorem{problem}{Problem}[section]
%\newtheorem{proposition}{Proposition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{assumption}{Assumption}
\newtheorem{setting}{Setting}
%\newtheorem{solution}{Solution}[section]
%\newtheorem{summary}{Summary}[section]



\newcommand{\hvx}{{\hat{\vx}}}
\DeclarePairedDelimiter{\dotp}{\langle}{\rangle} 
